Verification of the Tree-Based Hierarchical Read-Copy Update in the Linux Kernel

Read-Copy Update (RCU) is a scalable, high-performance Linux-kernel synchronization mechanism that runs low-overhead readers concurrently with updaters. Production-quality RCU implementations for multi-core systems are decidedly non-trivial. Giving the ubiquity of Linux, a rare "million-year" bug can occur several times per day across the installed base. Stringent validation of RCU's complex behaviors is thus critically important. Exhaustive testing is infeasible due to the exponential number of possible executions, which suggests use of formal verification. Previous verification efforts on RCU either focus on simple implementations or use modeling languages, the latter requiring error-prone manual translation that must be repeated frequently due to regular changes in the Linux kernel's RCU implementation. In this paper, we first describe the implementation of Tree RCU in the Linux kernel. We then discuss how to construct a model directly from Tree RCU's source code in C, and use the CBMC model checker to verify its safety and liveness properties. To our best knowledge, this is the first verification of a significant part of RCU's source code, and is an important step towards integration of formal verification into the Linux kernel's regression test suite.

==> Makefile <==
TARGET = paper
DEPS = intro.tex background.tex api_usage.tex tree_rcu.tex api_impl.tex callback.tex \
       data_structure.tex quiescent_state_detection.tex grace_period_detection.tex \
       running_example.tex modeling.tex experiments.tex bug_cases.tex cbmc.tex \
       results_cbmc.tex results_run.tex related_work.tex concl.tex barchart_*.tex \

CLASSFILE = 
BIBFILE = paper.bib

SOURCE_FILE = $(TARGET).tex

LATEX = pdflatex
BIBTEX = bibtex

all: $(TARGET).pdf

$(CLASSFILE):

$(BIBFILE):

$(TARGET).pdf: $(SOURCE_FILE) $(DEPS) $(CLASSFILE) $(BIBFILE)
	$(LATEX) $(SOURCE_FILE)
	$(BIBTEX) $(TARGET)
	while ( \
		$(LATEX) $(TARGET) ; \
		grep "Rerun to get" $(TARGET).log > /dev/null \
	) do true ; done

clean:
	rm -f $(TARGET).aux $(TARGET).bbl $(TARGET).blg $(TARGET).log 

allclean: clean
	rm -f $(TARGET).pdf


